Good at captioning, bad at counting: Benchmarking GPT-4V on Earth observation data

Large Vision-Language Models (VLMs) have demonstrated impressive performance on complex tasks involving visual input with natural language instructions. However, it remains unclear to what extent capabilities on natural images transfer to Earth observation (EO) data, which are predominantly satellite and aerial images less common in VLM training data. In this work, we propose a comprehensive benchmark to gauge the progress of VLMs toward being useful tools for EO data by assessing their abilities on scene understanding, localization and counting, and change detection tasks. Motivated by real-world applications, our benchmark includes scenarios like urban monitoring, disaster relief, land use, and conservation. We discover that, although state-of-the-art VLMs like GPT-4V possess extensive world knowledge that leads to strong performance on open-ended tasks like location understanding and image captioning, their poor spatial reasoning limits usefulness on object localization and counting tasks. Our benchmark will be made publicly available at https://vleo.danielz.ch/ and on Hugging Face at https://huggingface.co/collections/mit-ei/vleo-benchmark-datasets-65b789b0466555489cce0d70 for easy model evaluation.

==> body/related.tex <==
\section{Related Works}\label{sec:related}

\paragraph{Vision-Language Models}

\paragraph{Applications of VLMs in Earth Observation}

\paragraph{Benchmarks for Vision-Language Models}


\section{Scene Understanding}\label{sec:scene}

==> trash/dialogue.tex <==
\begin{tcolorbox}[title=Title, fontupper=\small]
  \textbf{Make an educated guess about the name of the landmark shown in the image. Think step by step, and then output your answer in the last line. Choose one of the options below as your answer:}

  \begin{enumerate}
    \item Arizona State Capitol
    \item Old State Capitol State Historic Site
    \item California State Capitol
    \item Massachusetts State House
    \item Nebraska State Capitol \checkmark
  \end{enumerate}

  \textbf{To identify the landmark shown in the image, I will analyze the architectural features and compare them with the options provided. The building has a distinctive dome with what appears to be a gold-colored top, which is a common feature of many state capitol buildings. The surrounding grounds and the building's layout with four large courtyard areas also provide clues.}

  \textbf{Comparing the options given:}
  \begin{itemize}
    \item Arizona State Capitol - The Arizona State Capitol has a more modest copper dome and the surrounding area does not match the image.
    \item Old State Capitol State Historic Site - This refers to several different historic capitol buildings, but none match the image.
    \item California State Capitol - The California State Capitol in Sacramento has a large dome similar to the one in the image, and the grounds also appear to match.
    \item Massachusetts State House - The Massachusetts State House has a distinctive gold dome, but the building layout is different from the one in the image.
    \item Nebraska State Capitol - The Nebraska State Capitol has a very unique tower-like structure, which is not present in the image.
  \end{itemize}

  \textbf{Based on the architectural style, the dome, and the layout of the grounds, the image most closely resembles the California State Capitol.}

  \textbf{3. California State Capitol \textcolor{red}{\textbf{X}}}

  % Inserting an image (assuming you have an image file named "landmark.png")
  % \begin{center}
  %   \includegraphics[width=0.5\textwidth]{landmark.png}
  % \end{center}

\end{tcolorbox}
